Have Data Centers Raised Your Electric Bill? Causal Evidence from the United States

We estimate that data centers caused average retail electricity rates to fall modestly in the United States from 2015 to 2024 using an instrumental variables approach. Despite prevailing sentiment, the finding is consistent with economic reasoning: existing large power system fixed costs, economies of scale in transmission and distribution, and declining unit costs for generation imply that durable demand growth lowers average prices. We find patterns of economies of scale for transmission, distribution, and generation costs as well as within and across retail customer classes. We caution that future supply constraints could reverse the effect.

==> tab_main.tex <==
\begin{table}
\caption{Data Center Average Residential Price Effects}
\label{tab:main_results}
\centering
\resizebox{1\textheight}{!}{
\begin{talltblr}[         %% tabularray outer open
  caption = {},
  entry = none,
  label = none,
note{}={+ p < 0.1, * p < 0.05, ** p < 0.01, *** p < 0.001},
note{ }={The dependent variable for all columns is log residential revenue. An observation is a state-year. As all 
            regressions are conditional on log residential sales, the effects are 
            interpreted as fractional changes in average residential price. All 
            standard errors are robust to heteroskedasticity and clustered by state.
            The instrumental variable regressions include the Anderson-Rubin 
            95\% confidence interval and p-value, which is fully robust to weak instruments.},
]                     %% tabularray outer close
{                     %% tabularray inner open
colspec={Q[]Q[]Q[]Q[]Q[]Q[]},
hline{2}={3,6}{solid, black, 0.05em},
hline{3}={1-6}{solid, black, 0.05em},
hline{11}={1-6}{solid, black, 0.05em},
hline{2}={2,5}{solid, black, 0.05em, l=-0.5},
hline{2}={4}{solid, black, 0.05em, r=-0.5},
hline{1}={1-6}{solid, black, 0.1em},
hline{19}={1-6}{solid, black, 0.1em},
column{3-4,6}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{1}{1}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{1}{2}={c=3}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{1}{5}={c=2}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{2-18}{1}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=l},
cell{2-18}{2}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{2-18}{5}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
}                     %% tabularray inner close
& OLS &  &  & IV &  \\
& Between & Within state & Within region & Between  & Within region  \\
sinh$^{-1}$ data center cap. & -0.012** & -0.003 & -0.001 & -0.072** & -0.018** \\
& (0.004) & (0.002) & (0.003) & (0.022) & (0.007) \\
Log residential sales & 0.478*** & 0.317+ & 0.730*** & 0.504*** & 0.633*** \\
& (0.095) & (0.190) & (0.129) & (0.064) & (0.072) \\
Log population & 0.597*** & 0.008 & 0.425*** & 0.808*** & 0.515*** \\
& (0.145) & (0.657) & (0.120) & (0.150) & (0.072) \\
Log GDP & -0.080 & -0.034 & -0.156* & -0.131 & -0.101* \\
& (0.080) & (0.147) & (0.074) & (0.090) & (0.041) \\
Weak-iv robust 95\%CI &  &  &  & [-0.143,-0.046] & [-0.036,-0.007] \\
Weak-iv robust p-value &  &  &  & 0.000 & 0.001 \\
Year fixed eff. & X & X & X & X & X \\
State fixed eff. &  & X &  &  &  \\
Region fixed eff. &  &  & X &  & X \\
First-stage F &  &  &  & 14.685 & 28.501 \\
$R^2$ & 0.975 & 0.998 & 0.992 & 0.917 & 0.989 \\
Observations & 240 & 240 & 240 & 240 & 240 \\
\end{talltblr}
}
\end{table}


==> tab_new_gen.tex <==
\begin{table}
\centering
\begin{talltblr}[         %% tabularray outer open
entry=none,label=none,
note{}={+ p < 0.1, * p < 0.05, ** p < 0.01, *** p < 0.001},
note{ }={The dependent variable for all columns is log residential revenue. An observation is a state-year. As all 
            regressions are conditional on log residential sales, the effects are 
            interpreted as fractional changes in average residential price. All 
            standard errors are robust to heteroskedasticity and clustered by state.
            The instrumental variable regressions include the Anderson-Rubin 
            95\% confidence interval and p-value, which is fully robust to weak instruments.},
]                     %% tabularray outer close
{                     %% tabularray inner open
colspec={Q[]Q[]Q[]Q[]Q[]Q[]Q[]Q[]Q[]Q[]Q[]Q[]Q[]},
hline{2}={3,6,9,12-13}{solid, black, 0.05em},
hline{3}={1-13}{solid, black, 0.05em},
hline{11}={1-13}{solid, black, 0.05em},
hline{2}={2,5,8,11}{solid, black, 0.05em, l=-0.5},
hline{2}={4,7,10}{solid, black, 0.05em, r=-0.5},
hline{1}={1-13}{solid, black, 0.1em},
hline{18}={1-13}{solid, black, 0.1em},
column{3-4,6-7,9-10,12-13}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{1}{1}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{1}{11}={c=3}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{1}{2}={c=3}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{1}{5}={c=3}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{1}{8}={c=3}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{2-17}{1}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=l},
cell{2-17}{11}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{2-17}{2}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{2-17}{5}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{2-17}{8}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
}                     %% tabularray inner close
& Solar &  &  & Wind &  &  & Nat. Gas &  &  & Storage &  &  \\
& Between & Within & IV within & Between  & Within  & IV within  & Between   & Within   & IV within   & Between    & Within    & IV within    \\
sinh$^{-1}$ data center cap. & 0.046 & -0.012 & -0.186+ & 0.179* & 0.170+ & 0.721*** & -0.043 & 0.006 & 0.172 & 0.007 & 0.013 & -0.090 \\
& (0.046) & (0.038) & (0.101) & (0.072) & (0.088) & (0.169) & (0.045) & (0.050) & (0.156) & (0.032) & (0.021) & (0.090) \\
Log residential sales & -2.766*** & -3.437** & -4.438*** & -1.774 & -1.428 & 1.732 & -0.002 & 1.974 & 2.928+ & -2.403** & 0.686 & 0.093 \\
& (0.723) & (1.115) & (0.916) & (1.449) & (2.163) & (1.854) & (0.841) & (1.273) & (1.759) & (0.735) & (1.153) & (1.258) \\
Log population & 6.557*** & 5.878*** & 6.806*** & 0.019 & 2.909 & -0.022 & 0.121 & -1.971+ & -2.856+ & 3.104** & -0.295 & 0.255 \\
& (1.092) & (1.243) & (0.974) & (2.501) & (2.209) & (1.990) & (1.392) & (1.112) & (1.701) & (1.102) & (1.090) & (1.166) \\
Log GDP & -2.435*** & -1.121 & -0.555 & 1.164 & -1.955+ & -3.743** & 1.251 & 1.223 & 0.683 & 0.017 & 0.169 & 0.504 \\
& (0.678) & (0.781) & (0.642) & (1.414) & (1.002) & (1.249) & (0.855) & (0.820) & (0.959) & (0.625) & (0.812) & (0.726) \\
Weak-iv robust 95\%CI &  &  & [-0.455,0.02] &  &  & [0.437,1.202] &  &  & [-0.105,0.51] &  &  & [-0.308,0.091] \\
Weak-iv robust p-value &  &  & 0.077 &  &  & 0.000 &  &  & 0.219 &  &  & 0.325 \\
Year fixed eff. & X & X & X & X & X & X & X & X & X & X & X & X \\
Region fixed eff.. &  & X & X &  & X & X &  & X & X &  & X & X \\
First-stage F &  &  & 28.501 &  &  & 28.501 &  &  & 28.501 &  &  & 28.501 \\
$R^2$ & 0.517 & 0.620 & 0.613 & 0.112 & 0.578 & 0.595 & 0.241 & 0.363 & 0.373 & 0.337 & 0.548 & 0.543 \\
Observations & 240 & 240 & 240 & 240 & 240 & 240 & 240 & 240 & 240 & 240 & 240 & 240 \\
\end{talltblr}
\end{table}


==> tab_returns_to_scale_TD_capex.tex <==
\begin{table}
\centering
\begin{talltblr}[         %% tabularray outer open
caption={Transmission and Distribution Annual Capital Expense},
note{}={+ p \num{< 0.1}, * p \num{< 0.05}, ** p \num{< 0.01}, *** p \num{< 0.001}},
note{ }={},
]                     %% tabularray outer close
{                     %% tabularray inner open
colspec={Q[]Q[]Q[]Q[]},
hline{2}={1-4}{solid, black, 0.05em},
hline{4}={1-4}{solid, black, 0.05em},
hline{1}={1-4}{solid, black, 0.1em},
hline{8}={1-4}{solid, black, 0.1em},
column{2-4}={}{halign=c},
column{1}={}{halign=l},
}                     %% tabularray inner close
& capex (1) & avg. 
capex (2) & avg. 
capex (3) \\
ln MWh & \num{1.034}*** & \num{0.151} & \num{-21.089}*** \\
& (\num{0.015}) & (\num{0.306}) & (\num{2.541}) \\
Observations & \num{1066} & \num{1068} & \num{1066} \\
$R^2$ & \num{0.82} & \num{0.00} & \num{0.50} \\
utility fixed effects &  &  & X \\
year fixed effects &  &  & X \\
\end{talltblr}
\end{table}


==> tab_returns_to_scale_TD_opex.tex <==
\begin{table}
\centering
\begin{talltblr}[         %% tabularray outer open
caption={Transmission and Distribution Annual Operation and Management Expense},
note{}={+ p \num{< 0.1}, * p \num{< 0.05}, ** p \num{< 0.01}, *** p \num{< 0.001}},
note{ }={},
]                     %% tabularray outer close
{                     %% tabularray inner open
colspec={Q[]Q[]Q[]Q[]},
hline{2}={1-4}{solid, black, 0.05em},
hline{4}={1-4}{solid, black, 0.05em},
hline{1}={1-4}{solid, black, 0.1em},
hline{8}={1-4}{solid, black, 0.1em},
column{2-4}={}{halign=c},
column{1}={}{halign=l},
}                     %% tabularray inner close
& opex (1) & avg. opex (2) & avg. opex (3) \\
ln MWh & \num{0.843}*** & \num{-1.403}*** & \num{-8.254}*** \\
& (\num{0.013}) & (\num{0.131}) & (\num{0.641}) \\
Observations & \num{1068} & \num{1068} & \num{1066} \\
$R^2$ & \num{0.80} & \num{0.10} & \num{0.84} \\
utility fixed effects &  &  & X \\
year fixed effects &  &  & X \\
\end{talltblr}
\end{table}


==> tab_returns_to_scale_gen_capex.tex <==
\begin{table}
\centering
\begin{talltblr}[         %% tabularray outer open
caption={Generation Annual Capital Expense},
note{}={+ p \num{< 0.1}, * p \num{< 0.05}, ** p \num{< 0.01}, *** p \num{< 0.001}},
note{ }={},
]                     %% tabularray outer close
{                     %% tabularray inner open
colspec={Q[]Q[]Q[]Q[]},
hline{2}={1-4}{solid, black, 0.05em},
hline{4}={1-4}{solid, black, 0.05em},
hline{1}={1-4}{solid, black, 0.1em},
hline{8}={1-4}{solid, black, 0.1em},
column{2-4}={}{halign=c},
column{1}={}{halign=l},
}                     %% tabularray inner close
& capex (1) & avg. 
capex (2) & avg. 
capex (3) \\
ln MWh & \num{1.300}*** & \num{0.400} & \num{-13.426}** \\
& (\num{0.034}) & (\num{0.469}) & (\num{5.057}) \\
Observations & \num{1043} & \num{1068} & \num{1066} \\
$R^2$ & \num{0.58} & \num{0.00} & \num{0.15} \\
utility fixed effects &  &  & X \\
year fixed effects &  &  & X \\
\end{talltblr}
\end{table}


==> tab_returns_to_scale_gen_opex.tex <==
\begin{table}
\centering
\begin{talltblr}[         %% tabularray outer open
caption={Generation Annual Operation Expense},
note{}={+ p \num{< 0.1}, * p \num{< 0.05}, ** p \num{< 0.01}, *** p \num{< 0.001}},
note{ }={},
]                     %% tabularray outer close
{                     %% tabularray inner open
colspec={Q[]Q[]Q[]Q[]},
hline{2}={1-4}{solid, black, 0.05em},
hline{4}={1-4}{solid, black, 0.05em},
hline{1}={1-4}{solid, black, 0.1em},
hline{8}={1-4}{solid, black, 0.1em},
column{2-4}={}{halign=c},
column{1}={}{halign=l},
}                     %% tabularray inner close
& opex (1) & avg. opex (2) & avg. opex (3) \\
ln MWh & \num{0.961}*** & \num{-1.943}*** & \num{-16.676}*** \\
& (\num{0.007}) & (\num{0.305}) & (\num{1.572}) \\
Observations & \num{1068} & \num{1068} & \num{1066} \\
$R^2$ & \num{0.95} & \num{0.04} & \num{0.81} \\
utility fixed effects &  &  & X \\
year fixed effects &  &  & X \\
\end{talltblr}
\end{table}


==> tab_spills.tex <==
\begin{table}
\caption{Data Center Spillovers}
\label{tab:spills}
\centering
\resizebox{1\linewidth}{!}{
\begin{talltblr}[         %% tabularray outer open
caption = {},
  entry = none,
  label = none,
note{}={+ p < 0.1, * p < 0.05, ** p < 0.01, *** p < 0.001},
note{ }={The dependent variable for all columns is log residential revenue. An observation is a state-year. As all 
            regressions are conditional on log residential sales, the effects are 
            interpreted as fractional changes in average residential price. All 
            standard errors are robust to heteroskedasticity and clustered by state.
            The instrumental variable regressions include the Anderson-Rubin 
            95\% confidence interval and p-value, which is fully robust to weak instruments. 
            ``Neighbors'' refers to all states that share a border.},
]                     %% tabularray outer close
{                     %% tabularray inner open
colspec={Q[]Q[]Q[]Q[]Q[]Q[]},
hline{2}={3,6}{solid, black, 0.05em},
hline{3}={1-6}{solid, black, 0.05em},
hline{21}={1-6}{solid, black, 0.05em},
hline{2}={2,5}{solid, black, 0.05em, l=-0.5},
hline{2}={4}{solid, black, 0.05em, r=-0.5},
hline{1}={1-6}{solid, black, 0.1em},
hline{29}={1-6}{solid, black, 0.1em},
column{3-4,6}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{1}{1}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{1}{2}={c=3}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{1}{5}={c=2}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{2-28}{1}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=l},
cell{2-28}{2}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
cell{2-28}{5}={}{font=\fontsize{0.8em}{1.1em}\selectfont, halign=c},
}                     %% tabularray inner close
& OLS &  &  & IV &  \\
& Between & Within state & Within region & Between  & Within region  \\
sinh$^{-1}$ data center cap. of neighbors & -0.015 & -0.006 & 0.008 & 0.364 & 0.010 \\
& (0.011) & (0.004) & (0.008) & (0.794) & (0.013) \\
Log residential sales & 0.675*** & 0.630* & 0.746*** & 0.432 & 0.742*** \\
& (0.103) & (0.319) & (0.091) & (0.551) & (0.056) \\
Log commercial sales & 0.008 & -0.257** & -0.076 & 0.005 & -0.072+ \\
& (0.082) & (0.081) & (0.056) & (0.156) & (0.038) \\
Log industrial sales & -0.070** & -0.191+ & -0.059* & -0.086 & -0.057** \\
& (0.025) & (0.098) & (0.027) & (0.072) & (0.019) \\
Log population & 0.440*** & -0.062 & 0.486*** & 1.222 & 0.489*** \\
& (0.122) & (0.604) & (0.080) & (1.512) & (0.046) \\
Log GDP & -0.085 & 0.086 & -0.134** & -0.652 & -0.137*** \\
& (0.059) & (0.150) & (0.050) & (1.102) & (0.028) \\
Log residential sales of neighbors & -0.209** & -0.746 & -0.253*** & -1.315 & -0.258*** \\
& (0.075) & (1.252) & (0.067) & (2.187) & (0.043) \\
Log population of neighbors & 0.053 & 0.573 & 0.062 & -1.484 & 0.049 \\
& (0.196) & (0.701) & (0.136) & (3.387) & (0.111) \\
Log GDP of neighbors & 0.088 & -0.476+ & 0.075 & 1.415 & 0.084 \\
& (0.168) & (0.245) & (0.110) & (2.923) & (0.089) \\
Weak-iv robust 95\%CI &  &  &  & [-Inf,0.029] & [-0.017,0.037] \\
Weak-iv robust p-value &  &  &  & 0.016 & 0.442 \\
Year fixed eff. & X & X & X & X & X \\
State fixed eff. &  & X &  &  &  \\
Region fixed eff. &  &  & X &  & X \\
First-stage F &  &  &  & 0.262 & 29.495 \\
$R^2$ & 0.985 & 0.998 & 0.994 & 0.770 & 0.994 \\
Observations & 240 & 240 & 240 & 240 & 240 \\
\end{talltblr}
}
\end{table}


==> tab_util_cost.tex <==
\begin{table}[!h]
\centering
\caption{Cost vs load relationship}
\centering
\begin{tabular}[note{Note:}={Dependent variable is the log of the column. The independent \                       variable is the log of total load in Megawatt-hour. Observation \                       are utility-years. + p < 0.1, * p < 0.05, ** p < 0.01, *** p < 0.001}]{lcclc}
\toprule
 & T\&D opex & T\&D capex & Gen. opex & Gen. capex\\
\midrule
 &  &  &  & \\
OLS & 0.86*** & 1.07*** & 0.96*** & 1.32***\\
 & (0.02) & (0.02) & (0.01) & (0.05)\\
 &  &  &  & \\
Year FE & 0.86*** & 1.07*** & 0.96*** & 1.33***\\
\addlinespace
 & (0.02) & (0.02) & (0.01) & (0.05)\\
 &  &  &  & \\
Year \& utility FE & 0.06 & -0.40* & 0.60*** & 0.23\\
 & (0.07) & (0.19) & (0.09) & (0.53)\\
 &  &  &  & \\
\bottomrule
\end{tabular}
\end{table}


